Attention Speaks Volumes: Localizing and Mitigating Bias in Language Models

We explore the internal mechanisms of how bias emerges in large language models (LLMs) when provided with ambiguous comparative prompts: inputs that compare or enforce choosing between two or more entities without providing clear context for preference. Most approaches for bias mitigation focus on either post-hoc analysis or data augmentation. However, these are transient solutions, without addressing the root cause: the model itself. Numerous prior works show the influence of the attention module towards steering generations. We believe that analyzing attention is also crucial for understanding bias, as it provides insight into how the LLM distributes its focus across different entities and how this contributes to biased decisions. To this end, we first introduce a metric to quantify the LLM's preference for one entity over another. We then propose $\texttt{ATLAS}$ (Attention-based Targeted Layer Analysis and Scaling), a technique to localize bias to specific layers of the LLM by analyzing attention scores and then reduce bias by scaling attention in these biased layers. To evaluate our method, we conduct experiments across 3 datasets (BBQ, Crows-Pairs, and WinoGender) using $\texttt{GPT-2 XL}$ (1.5B), $\texttt{GPT-J}$ (6B), $\texttt{LLaMA-2}$ (7B) and $\texttt{LLaMA-3}$ (8B). Our experiments demonstrate that bias is concentrated in the later layers, typically around the last third. We also show how $\texttt{ATLAS}$ effectively mitigates bias through targeted interventions without compromising downstream performance and an average increase of only 0.82% in perplexity when the intervention is applied. We see an average improvement of 0.28 points in the bias score across all the datasets.

==> Tables/Pasta.tex <==
\setlength{\tabcolsep}{2pt} % Reduce column spacing
\renewcommand{\arraystretch}{0.9} % Reduce row height

\begin{table}[h!]
\centering
\begin{tabular}{@{}l|>{\centering\arraybackslash}p{1.4cm} >{\centering\arraybackslash}p{1.4cm}@{}}
\toprule
\multirow{2}{*}{\textbf{Bias Category}} & \multicolumn{2}{c}{\texttt{GPT-J}} \\
\cmidrule(lr){2-3}
& \textbf{\fontsize{7}{12}\selectfont $\Delta \text{EBS}_{\text{PASTA}}$} & \textbf{\fontsize{7}{12}\selectfont $\Delta \text{EBS}_\name$} \\
\midrule
Age                      &  0.278   & 0.437    \\
Disability Status        &  0.158   & 0.166    \\
Gender Identity          &  0.182   & 0.375    \\
Nationality              &  0.217   & 0.371    \\
Physical Appearance      &  0.209   & 0.314    \\
Race/Ethnicity           &  0.232   & 0.317    \\
Race/Gender              &  0.143   & 0.279    \\
Race/SES                 &  0.130   & 0.254    \\
Religion                 &  0.097   & 0.151    \\
Sexual Orientation       &  0.157   & 0.221    \\
SES                      &  0.344   & 0.354    \\
\bottomrule
\end{tabular}
\caption{\footnotesize {\bf Increase in EBS} for \texttt{GPT-J} using \textsc{Pasta} vs \name\ with respect to the base model for BBQ.}
\vspace{-5pt}
\label{tab:5}
\end{table}

